PathStream: Towards Streaming Diagnostic Copilots for Whole-Slide Pathology

Pathologists reach a diagnosis by integrating morphological evidence across regions and magnifications along viewing trajectories. Existing pathology AI rarely reflects this process: models predict from selected image regions, answer questions within fixed visual contexts, or navigate slides autonomously. We formalize pathologist-led streaming diagnosis, in which the pathologist controls navigation while a copilot selectively describes incoming views and synthesizes accumulated evidence into a final diagnosis. We record five pathologists' viewing trajectories on 1,791 TCGA whole-slide images (WSIs) spanning ten organs, with response labels, morphological descriptions, and session-level findings and diagnoses. We construct PathStreamBench to assess response timing, morphological description, and session-level diagnosis, alongside auxiliary video understanding. We introduce PathStream, which jointly learns streaming responses and diagnosis through two-stage training, with a diagnosis-attention loss guiding attention during diagnosis to relevant visual and textual evidence accumulated as the examination unfolds. PathStream outperforms 14 vision-language models and three domain-fine-tuned baselines on the core tasks, achieving a trajectory WSI Relevance score of 77.87, surpassing the strongest domain-fine-tuned baseline's 62.76. Without additional training, its diagnostic capabilities generalize to new educational pathology videos, three external centers, and an unseen organ.

==> Makefile <==
.PHONY: pdf

pdf:
	@build_dir=$$(mktemp -d /tmp/pathstream-arxiv.XXXXXX); \
	latexmk -pdf -interaction=nonstopmode -halt-on-error -outdir="$$build_dir" main.tex && \
	cp "$$build_dir/main.pdf" main.pdf && \
	rm -r "$$build_dir"
	@pdfinfo main.pdf | awk '/^Pages:|^Page size:|^File size:/'
	@pdffonts main.pdf

